Convex Influences

We introduce a new notion of influence for symmetric convex sets over Gaussian space, which we term "convex influence". We show that this new notion of influence shares many of the familiar properties of influences of variables for monotone Boolean functions $f: \{\pm1\}^n \to \{\pm1\}.$ Our main results for convex influences give Gaussian space analogues of many important results on influences for monotone Boolean functions. These include (robust) characterizations of extremal functions, the Poincar\'e inequality, the Kahn-Kalai-Linial theorem, a sharp threshold theorem of Kalai, a stability version of the Kruskal-Katona theorem due to O'Donnell and Wimmer, and some partial results towards a Gaussian space analogue of Friedgut's junta theorem. The proofs of our results for convex influences use very different techniques than the analogous proofs for Boolean influences over $\{\pm1\}^n$. Taken as a whole, our results extend the emerging analogy between symmetric convex sets in Gaussian space and monotone Boolean functions from $\{\pm1\}^n$ to $\{\pm1\}$

==> sections/prelims-longer.tex <==
%!TEX root = ../main.tex

\section{Preliminaries} \label{sec:prelims}

In this section we give preliminaries setting notation and recalling useful background on convex geometry, log-concave functions, and Hermite analysis over $\calN\pbra{0, \sigma^2}^n$.

\subsection{Convex Geometry}

Below we briefly recall some basic facts and notation from convex geometry and log-concavity that we will use. Some of our main results employ relatively sophisticated results from these areas; we will recall these as necessary in the relevant sections and here record only basic facts.\ignore{ (for example, the $S$-inequality of Lata\l a and Oleskiewicz \cite{s-inequality} is crucial to the main results of \Cref{sec:poincare-kkl}),}  For a general and extensive resource we refer the interested reader to \cite{aga-book}. 

We identify sets $K \sse \R^n$ with their indicator functions $K : \R^n \to \zo$, and we say that $K\sse\R^n$ is \emph{symmetric} if $K(x) = K(-x)$. We write $B_r$ to denote the origin-centered ball of radius $r$ in $\R^n$.  If $K \subseteq \R^n$ is a nonempty symmetric convex set then we let $\rinn(K)$ denote $\sup_{r \geq 0} \{r: B_r \subseteq K\}$ and we refer to this as the \emph{in-radius} of $K$. We record the following easy consequence of the separating hyperplane theorem:\rnote{I think we are likely to use this somewhere, right?}

\begin{fact} \label{fact:slab}
Let $K \subseteq \R^n$ be a symmetric convex set with in-radius $\rinn < \infty.$ Then there is a direction $v \in \mathbb{S}^{n-1}$ such that $K \subseteq \{x \in \R^n: |v \cdot x| \leq \rinn\}.$
\end{fact}


Recall that a function $f : \R^n \to \R_{\geq 0}$ is \emph{log-concave} if its domain is a convex set and it satisfies $f(\theta x + (1-\theta)y) \geq f(x)^\theta f(y)^{1-\theta}$ for all $x, y \in \mathrm{domain}(f)$ and $\theta \in [0,1]$. In particular, the $0/1$-indicator functions of convex sets are log-concave. 

Recall that the \emph{marginal} of  $f: \R^n \to \R$ on the set of variables $\{i_1,\dots,i_k\}$ is obtained by integrating out the other variables, i.e. it is the function
\[
g(x_{i_1},\dots,x_{i_k}) = \int_{\R^{n-k}} f(x_1,\dots,x_n) dx_{j_1} \dots dx_{j_{n-k}},
\]
where $\{j_{1},\dots,j_{n-k}\} = [n] \setminus \{i_1,\dots,i_k\}$.  We recall the following fact:
\begin{fact}[\cite{Dinghas,Leindler,Prekopa, Prekopa2} (see Theorem 5.1, \cite{LV07})] 
\label{fact:marginal-log-concave}
	All marginals of a log-concave function are log-concave.
\end{fact}
The next fact is obvious\rnote{is it obvious enough that we don't want to cite it? I guess we could cite \cite{Ibragimov:56} and/or \cite{An:95}} from the definition of log-concave functions. 
\begin{fact}
\label{fact:unimodal-log-concave}
	A one-dimensional log-concave function is unimodal. 
\end{fact}



\subsection{Hermite Analysis over $\calN\pbra{0, \sigma^2}^n$}

Our notation and terminology here follow Chapter~11 of \cite{ODbook}. We say that an $n$-dimensional \emph{multi-index} is a tuple $\alpha \in \N^n$, and we define 
\begin{equation} \label{eq:index-notation}
|\alpha| := \sum_{i=1}^n \alpha_i.
\end{equation}

We write $\calN(0, \sigma^2)^n$ to denote the $n$-dimensional Gaussian distribution with mean $0$ and variance $\sigma^2$, and denote the corresponding measure by $\gamma_{n, \sigma}(\cdot)$. When the dimension $n$ is clear from context we will simply write $\gamma_\sigma(\cdot)$ instead, and sometimes when $\sigma=1$ we simply write $\gamma$ for $\gamma_{1}$. For $n \in \N_{> 0}$, we write $L^2\pbra{\R^n, \gamma_{\sigma}}$ to denote the space of functions $f: \R^n \to \R$ that have finite second moment $\|f\|_2^2$ under the Gaussian measure $\gamma_\sigma$, that is: 
\[
\|f\|_2^2 = \Ex_{\bz \sim \calN\pbra{0, \sigma^2}^n} \left[f(\bz)^2\right]^{1/2} < \infty.
\]
We view $L^2\pbra{\R^n, \gamma_\sigma}$ as an inner product space with $\la f, g \ra := \E_{\bz \sim \calN\pbra{0,\sigma^2}^n}[f(\bz)g(\bz)]$ for $f, g \in L^2\pbra{\R^n, \gamma_\sigma}$. 

Recall the \emph{Hermite basis} for $1$-dimensional Gaussian space $L^2\pbra{\R, \gamma_{1}}$:

\begin{definition}[Hermite basis]
	The \emph{Hermite polynomials} $(h_j)_{j\in\N}$ are the univariate polynomials defined as
	$$h_j(x) = \frac{(-1)^j}{\sqrt{j!}} \exp\left(\frac{x^2}{2}\right) \cdot \frac{d^j}{d x^j} \exp\left(-\frac{x^2}{2}\right).$$
\end{definition}


\begin{fact} [Proposition~11.33, \cite{ODbook}] \label{fact:hermite-orthonormality}
	The Hermite polynomials $(h_j)_{j\in\N}$ form a complete, orthonormal basis for $L^2(\R, \gamma_1)$. For $n > 1$ the collection of $n$-variate polynomials given by $(h_\alpha)_{\alpha\in\N^n}$ where
	$$h_\alpha(x) := \prod_{i=1}^n h_{\alpha_i}(x)$$
	forms a complete, orthonormal basis for $L^2(\R^n, \gamma_{n,1})$. 
\end{fact}

We will also require an orthonormal basis for $L^2\pbra{\R, \gamma_\sigma}$. 

\begin{definition}[$\sigma$-biased Hermite polynomials] \label{def:biased-hermite-basis}
	Given $\sigma > 0$, we define the \emph{$\sigma$-biased $i^\text{th}$ Hermite polynomial} $h_{i, \sigma}(x)$ as
\[h_{i,\sigma}(x) := h_i\pbra{\frac{x}{\sigma}}\]
where $h_i$ denotes the $i^\text{th}$ univariate Hermite polynomial. 
\end{definition}

\begin{claim} \label{claim:biased-hermite-orthonormal}
	The polynomials $(h_{i, \sigma})_{i\in\N}$ are orthonormal with respect to $L^2\pbra{\R, \gamma_\sigma}$. 
\end{claim}

\begin{proof}
	Indeed, we have
\begin{align*}
	\langle h_{i, \sigma},h_{j, \sigma} \rangle_{\gamma_{n, \sigma}} &= \int_{-\infty}^{\infty} h_i\pbra{\frac{x}{\sigma}} h_j\pbra{\frac{x}{\sigma}} {\frac 1 {\sigma \sqrt {2 \pi}}} e^{-x^2 / (2\sigma^2)} dx\\
	&=  \int_{-\infty}^{\infty} h_i(u) h_j(u) {\frac 1 {\sqrt{2 \pi}}} e^{-u^2/2} du \\
	&= \begin{cases}
		1 & i = j\\
		0 & i \neq j
	\end{cases}
\end{align*}
	where we made the substitution $u := \frac{x}{\sigma}$ and used the orthonormality of the Hermite basis with respect to $\gamma_{1}$ (see \Cref{fact:hermite-orthonormality}).
\end{proof}

As usual, we obtain an orthonormal basis for $L^2\pbra{\R^n, \gamma_{\sigma}}$ by taking $n$-fold products of the univariate polynomials:

\begin{fact} \label{fact:biased-hermite-orthonormality}
\ignore{The $\sigma$-biased Hermite polynomials $(h_{i,\sigma})_{i\in\N}$ form a complete, orthonormal basis for $L^2(\R, \gamma_1)$.}For $n \geq 1$ and $\sigma > 0$, the collection of $n$-variate $\sigma$-biased Hermite polynomials given by $(h_{\alpha, \sigma})_{\alpha\in\N^n}$ where
	$$h_{\alpha, \sigma}(x) := \prod_{i=1}^n h_{\alpha_i, \sigma}(x)$$
	forms a complete, orthonormal basis for $L^2(\R^n, \gamma_{n,\sigma})$. 
\end{fact}


Given a function $f \in L^2(\R^n, \gamma_\sigma)$ and $\alpha \in \N^n$, we define its \emph{($\sigma$-biased) Hermite coefficient on} $\alpha$ to be $\widetilde{f}_\sigma(\alpha) := \la f, h_{\alpha, \sigma} \ra$. It follows that $f$ is uniquely expressible as $f = \sum_{\alpha\in\N^n} \widetilde{f}_\sigma(\alpha)h_{\alpha, \sigma}$ with the equality holding in $L^2(\R^n, \gamma_\sigma)$; we will refer to this expansion as the \emph{Hermite expansion} of $f$. When $\sigma = 1$, we will simply write $\wt{f}(\alpha)$ instead of $\wt{f}_\sigma(\alpha)$ and $h_\alpha$ instead of $h_{\alpha, 1}$.
Parseval's and Plancharel's identities hold in this setting: 

\begin{fact}[Plancharel's identity] \label{fact:hermite-plancharel}
	For $f, g \in L^2(\R^n, \gamma_\sigma)$, we have:
	$$\la f, g\ra = \Ex_{\bz\sim\calN(0,\sigma^2)^n}[f(\bz)g(\bz)] = \sum_{\alpha\in \N^n}\widetilde{f}_\sigma(\alpha)\widetilde{g}_\sigma(\alpha),$$
	and as a special case we have Parseval's identity,
	$$\la f, f\ra = \Ex_{\bz\sim\calN(0,\sigma^2)^n}[f(\bz)^2] = \sum_{\alpha\in \N^n}\widetilde{f}_\sigma(\alpha)^2.$$ 
\end{fact}

The following notation will sometimes come in handy. 

\begin{definition} \label{def:hermite-coeff-along-direction}
	Let $v \in \mathbb{S}^{n-1}$ and $f \in L^2\pbra{\R^n, \gamma_\sigma}$. We define $f$'s \emph{Hermite coefficient of degree $k$ along $v$}, written $\wt{f}(kv)$, to be 
	\[\wt{f}_\sigma(kv) := \Ex_{\bx\sim\calN(0,\sigma^2)^n}\sbra{f(\bx)\cdot h_{k, \sigma}\pbra{v\cdot\bx}}.\]
\end{definition}

\begin{notation}
	We will write $e_i \in \N^n$ to denote the $i^\text{th}$ standard basis vector for $\R^n$, i.e. the unit vector with a 1 in coordinate $i$ and 0 in all other coordinates.
\ignore{
	\[(e_i)_j = \begin{cases}
 1 & i = j\\
 0 & i \neq j	
 \end{cases}.
\]}
\end{notation}

In this notation, for example, $\wt{f}(ke_i) = \E_{\bx\sim\calN(0,1)^n}\sbra{f(\bx)\cdot h_k(\bx_i)}$. 













